VizExtract: Automatic Relation Extraction from Data Visualizations

Visual graphics, such as plots, charts, and figures, are widely used to communicate statistical conclusions. Extracting information directly from such visualizations is a key sub-problem for effective search through scientific corpora, fact-checking, and data extraction. This paper presents a framework for automatically extracting compared variables from statistical charts. Due to the diversity and variation of charting styles, libraries, and tools, we leverage a computer vision based framework to automatically identify and localize visualization facets in line graphs, scatter plots, or bar graphs and can include multiple series per graph. The framework is trained on a large synthetically generated corpus of matplotlib charts and we evaluate the trained model on other chart datasets. In controlled experiments, our framework is able to classify, with 87.5% accuracy, the correlation between variables for graphs with 1-3 series per graph, varying colors, and solid line styles. When deployed on real-world graphs scraped from the internet, it achieves 72.8% accuracy (81.2% accuracy when excluding "hard" graphs). When deployed on the FigureQA dataset, it achieves 84.7% accuracy.

==> app-DatasetGeneration.tex <==
\section{Dataset Generation}

In order to accurately train and test our system, we need to generate many diverse graphs to use as training and testing data. In our system, we support the generation of graphs with varying numbers of series, colors and data styles. Furthermore, the types of series on each graph vary using a combination of scatter plots, line graphs, and bar graphs. These graphs are created in two stages: data generation and plotting.\par

For each graph type, the data is generated as follows. For scatter plots, we randomly choose a correlation ranging between -1 and 1. From this correlation we generate two series which have this correlation. Line graphs generate a line with slope ranging from -1 to 1 and a randomly varying y intercept. Each point of this data is then perturbed according to a normal distribution and then all of the data is plotted as a line. Bar graph data are created the same as line graph data except their y axes are adjusted so that are always non-zero. The perturbation is slightly exaggerated since variations are harder to see in data represented in the bar graph format. After creating the data, we record its correlation as calculated by the Spearman formula which returns a value ranging from -1 to 1. For all types of graphs, we use a threshold of 0.4, such that data with correlations above 0.4 are classified as positive correlation, those with correlations below -0.4 are classified as negative correlation, and those with correlations between -0.4 and 0.4 are classified as neutral correlation. This threshold of 0.4 is largely arbitrary. It was determined by visually analyzing graphs of different correlations to determine what levels of correlation looked visibly correlated in an attempt to mimic human assessment of the correlation of these graphs.

Once data is generated it then needs to be plotted. Each graph will consist of one to three series. However, before we can plot each graph, we need to determine the the plot style, the colors of each series of the data, and in the case of line graphs, the line style of each series of data. For each of these parameters, number of series, plot style, color, and line style, the choices of either fixed or randomly varying values are both permitted by the system and can be chosen according to the preferences desired by the given experiment. For parameters color and line style, when the system is set to the “random” setting, a parameter is chosen at random from an array of possible options. Once a color or line style is chosen, it is removed so that no two series in a single graph have the same color or line style. In the current model, the possible colors are red, green and blue and the possible line styles are solid, dotted, dashed, and dashes and dots alternating. Plot style applies to the entire graph, not just a single series so once all other parameters are set for all series, either a specific plot style is dictated by the experiment or is it is set to random, in which case a random plot style is selected from list of possible plot styles offered by \texttt{matplotlib}. Once these parameters have been determined, the graphs can be plotted and are ready to be used as training or testing data. See figure 2 for an example.\par

\begin{figure}
  \includegraphics[scale=0.5]{figures/example1.png}
  \caption{Example scatter plot graph with 3 series and multiple colors. \todo{I would add a few different plots with styles here}}
\end{figure}

==> app-experiments.tex <==
\section{Further Experiments}
\subsection{Impact of Design Choices}
\subsubsection{Test if preprocessing affects correct K choice}
A major component of our system is choosing the correct k value to use in k-means when segmenting out each series in the graph. This task essentially means determining how many series are present in the graph. Since all of the segmentation depends on a correctly chosen k, this step is very important. This experiment examine the importance of using our pre-processing algorithm on the k selection. To test this, we ran our pipeline to select k values with and without first preprocessing the images and compared them to manually labeled k values. We found that with the preprocessing this algorithm achieved $98\%$ accuracy and without it it was only able to get up to $22\%$ accuracy. Without preprocessing, we have lower accuracy here ($22\%$) than the overall system had before we implemented preprocessing since the current k selection algorithm relies on preprocessing to work. In contrast, the old CNN based k-selection algorithm did not rely on preprocessed images. We made the switch to preprocessing and the modified kneedle (k selection) algorithm for reasons outlined in experiment $3$.

\subsubsection{Test if preprocessing affects correct color segmentation from correct (manually selected) k choice}
This experiment highlights the importance of the preprocessing step in the pipeline. In our control condition, we do not perform any preprocessing and manually provide the correct k choice and then perform the segmentation step. In our intervention condition, we follow all of the same steps except we also preprocess the image before segmentation. In this experiment, we define accuracy as follows. \textbf{Accuracy} (max(num series - num errors) / num series): Control = 93.8, Intervention = 0. (Note: it is possible to lose more points than there are available to gain on a specific graph if you miss the correct series and report an incorrect one). In addition to this ``accuracy", we also measure the number of errors (on 50 graphs). \textbf{Errors}: Control = 109, Intervention = 3.

% \subsubsection{Test K current choice algorithm as compared to regular kneedle, CNN, SilScore}
% When tested on the synthetic graphs, the results are as follows: Modified Kneedle = 96\%, Regular kneedle = 53\%, CNN = 67\%. CNN result seems a little low, but still makes point that current is by far best, but that CNN is better than regular kneedle.


\subsubsection{Test the accuracy of the OCR on the results of the object detection network as opposed to just doing the OCR directly}
%\todoD{While this is nice to have, I am not sure if we need to have a whole experiment dedicated to showing this, might be able to just state that it is the case as we do earlier in the description}
This experiment shows the importance of the object detection network.
Our accuracy for axis information when using the object detection networks and then performing OCR on on specific identified areas resulted in 86\% accuracy.
Applying regular OCR over the entire image without any object detection resulted in 41\% accuracy on axis information.
From this result, we can conclude that object detection is essential to OCR accuracy.

% \subsubsection{Test current legend matching algorithm using medians and matching with minimum total distance vs naive matching of randomly pick a color match with closest and continue until all colors matched}
% \todoD{Not sure how important this one is}
% Both methods produced similar results when evaluated on the synthetic graphs. While this might seem to imply that the current matching algorithm is unnecessary, we could create a specific malicious example that could exist in the real world and where the current method would be far superior. Consider an image where the legend has different symbols for each series where some symbols are larger than others. Also consider that some legend strings might be longer than others. If the color of the largest symbol is selected first, then it could be closest to a long legend string that it is not actually paired with just because both are large making them closer in the horizontal direction enough such that their total distance is less than the true match. The current method tries all pairings and selects that matching that has the minimum total distance so in this scenario it would be guaranteed to try the true matching and then would select the true matching since the total distance would be less.

%Note: test this on both generated graphs and on wild dataset to see how they compare on both\\
%For generated graphs:\\
%Controls: regular kneedle, CNN, SilScore\\
%Predict current will be most accurate with CNN 2nd, reg needle 3rd, SilScore never return, too complex\\
%Results: Modified Kneedle = 96\%, Regular kneedle = 53\%, CNN = 67\%\\
%Notes: CNN result seems a little low, but still makes point that current is by far best, but that CNN is better than regular kneedle.\\
%Results show that as soon as you move to wild graphs, a network trained on generated graphs completely breaks down due to noise and diversity in graph data.


% Setup: 100 graphs generated in the default (matplotlib) style. Then use the two methods to determine the axis labels and graph titles of each graph. (not including legend since this also takes into account correlation and matching which is part of a different experiment)\\
% Control: train all styles test all styles\\
% Intervention: train just python style test all styles\\
% Hypothesis: training on all types will have significantly better accuracy on validation of all types\\
% Results: Control = 87\%, Intervention = 82.5\%

% try to determine how transferable it is to train on synthetic graphs. In our control condition, we train on wild graphs and test on wild graphs. In our intervention condition, we train on synthetically generated graphs and test on wild graphs. From this experiment we found that the control had 87\% accuracy and the intervention had 73\% accuracy. These results show that as expect training on the same type of data you are testing on is preferable, but that training on synthetic data only has a slight drop off.

==> app-preproc.tex <==
\section{More Details On Image Pre-Processing}
High saturation colors stand out and are easily differentiable to the human eye and thus graphs are often created with high saturation series (with different hues) such that these series can be easily differentiated by humans interpreting the graph. The algorithm works as follows: first we convert the entire image from RGB space to HSV space (hue, saturation, value). Then for each pixel in the image we threshold it by its saturation value. If the pixel's saturation is above the threshold, we set its saturation to the max possible (in openCV this corresponds to 255) and also set its value to the max value possible (255). If the pixel's saturation is below the threshold, we set its saturation to 0. After adjusting each pixel as such, we are left with an image where the highly saturated pixels are now the max saturation and value and pixels with low saturation now have saturation of $0$ which corresponds to white. Assuming a white background, with this method, all low saturation, gray-ish pixels will be converted to the white background color leaving only high saturation pixels. This method supports graphs with black backgrounds as it changes black backgrounds to white to match low sat pixels since shades near black have low saturation in OpenCV. This method also removes all intentionally gray pixels which is useful as many graphs have gray checkered backgrounds or gray solid backgrounds to help the reader, but that would confuse the network. Lastly, this method also removes grayscale axes automatically which eliminates the need for us to have to do so in the segmentation step with a rule-based approach that could be less general.

==> intro-old.tex <==


Data visualization is an important part of scientific communication. Visualizations convey complex relationships between variables in a cognitively-efficient way. While incredibly intuitive to humans, data represented in a visualization is inherently opaque to computers and can be considered dark data: data that is widely collected and stored but which cannot be interpreted by standard tools without human input. As such, the process of automatically extracting data from visualizations has a number of important and emerging applications.
Social media platforms such as Instagram employ manual fact checkers to identify potentially false or misleading content [cite]. However, automating this process would save both time and money as manual inspection of data is expensive and incredibly slow. Consider a social media company that wishes to determine whether infographics posted on the site constitute ``fake data’'. With a tool that can quickly and automatically extract the entities compared and high-level statistics from a plot, the company could compare these extracted relations against some ground truth data to automatically validate the accuracy of such infographics. This capability makes such a tool invaluable to identifying cases of implausible or misleading data.

% \todo{Read this paper: Extracting Databases from Dark Data with DeepDive, need a new paragraph in here setting up more of the context. Maybe mention Notebooks? Discuss}

While visualization extraction has many applications, in this paper, we follow the example of the application to iPython notebooks. These notebooks can contain code, text, plots, and are widely used on fields such as data science. Furthermore, these notebooks typically create their plots using python libraries such as matplotlib, the library used to generate the VizExtract synthetic dataset. A tool that could extract relationships from these plots would allow iPython notebooks hose graphs contain dark data, to be converted into interpretable data. Thus, data scientists using working with such notebooks would be able to gain access to a massive and valuable new set of “big data.”

\todo{Add citations. But overall pretty good}
There are many existing systems that attempt to extract data from plots (sometimes referred to as reverse engineering visualization). Some attempt to entirely reproduce the plot by extracting the individual data points, while others focus on more narrow and tractable tasks such as extracting solely the text from the plot. Given the ambitious nature of extracting the exact data points it is difficult to build a system that is robust to noise and messy data. On the other side of the spectrum, a system that can robustly extract text but has no data extraction capabilities is not especially helpful on its own either. Similarly, some systems support many plot formats, but only classify the plot types as opposed to actually extracting data from them. Others, provide robust and exhaustive extraction, but only for very specific plot types. Thus, it is important to balance robustness, widespread support, and the ability to perform useful data extraction.
This visualization extraction is mainly a computer vision problem. Many common 2D visualizations illustrate pairwise relationships between the visualized attributes. Most obviously, line charts and scatter plots have X-Y axes, but more subtly, a bar chart can be seen as relating a categorical or discrete attribute to a numerical one. From a chart, we can also learn about how the attributes are related, e.g., is there a positive correlation, or an exponential increase, or monotonicity, etc. 

As alluded to earlier, there are other frameworks that perform reverse engineering visualization [cite laundry list here], however, our model makes key contributions in its breadth of input types and robustness to noisy data. Other implementations are often specific to only a few graph types and do not always support multiple series in a single graph, whereas \sys is able to work more generally on most graph types and can support multiple series in the same graph (see table \_). Another major difference between \sys and these existing systems is that \sys performs “visual relation extraction” only looking at high level patterns in the data whereas the other existing systems all attempt to extract the exact input data. Deducing the precise input data from a visualization is often ill-posed because most visualizations are reductive (based on aggregation) and only contain data up-to pixel resolutions. However, even in situations where exact data extraction is feasible, determining these relations by VizExtract’s relation extraction method is much more robust. While any relation can be computed with the true data that would theoretically get extracted by any of these other systems, precise data extraction is inherently a more difficult problem and can be more sensitive to noisy or messy data. As such, exact data extraction can introduce errors that could alter the determined relation. Additionally, \sys is scalable to new relations (a feature also possessed by exact data extraction where any new relation can just be calculated from the retrieved data). In order to provide functionality for a new relation with \sys, one would simply add this relation to the synthetic graph labels and retrain the network.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/VizExtractDiagram.png}
    \caption{Conceptual overview of \sys}
    \label{fig:my_label}
\end{figure*}

